A Causal Mediation Model for Longitudinal Mediators and Survival Outcomes with an Application to Animal Behavior

In animal behavior studies, a common goal is to investigate the causal pathways between an exposure and outcome, and a mediator that lies in between. Causal mediation analysis provides a principled approach for such studies. Although many applications involve longitudinal data, the existing causal mediation models are not directly applicable to settings where the mediators are measured on irregular time grids. In this paper, we propose a causal mediation model that accommodates longitudinal mediators on arbitrary time grids and survival outcomes simultaneously. We take a functional data analysis perspective and view longitudinal mediators as realizations of underlying smooth stochastic processes. We define causal estimands of direct and indirect effects accordingly and provide corresponding identification assumptions. We employ a functional principal component analysis approach to estimate the mediator process, and propose a Cox hazard model for the survival outcome that flexibly adjusts the mediator process. We then derive a g-computation formula to express the causal estimands using the model coefficients. The proposed method is applied to a longitudinal data set from the Amboseli Baboon Research Project to investigate the causal relationships between early adversity, adult physiological stress responses, and survival among wild female baboons. We find that adversity experienced in early life has a significant direct effect on females' life expectancy and survival probability, but find little evidence that these effects were mediated by markers of the stress response in adulthood. We further developed a sensitivity analysis method to assess the impact of potential violation to the key assumption of sequential ignorability.

==> additionalreference.tex <==
Anderson, M. and M. Marmot. 2012. The effects of promotions on heart disease: Evidence from Whitehall. The Economic Journal 122:555-589.

Case, A. and C. Paxson. 2011. The long reach of childhood health and circumstance: evidence from the Whitehall II Study. The Economic Journal 121:F183-F204.

Chandola, T., M. Bartley, A. Sacker, C. Jenkinson, and M. Marmot. 2003. Health selection in the Whitehall II study, UK. Social Science & Medicine 56:2059-2072.

Chartier, M. J., J. R. Walker, and B. Naimark. 2010. Separate and cumulative effects of adverse childhood experiences in predicting adult health and health care utilization. Child Abuse & Neglect 34:454-464.

Elovainio, M., J. E. Ferrie, A. Singh-Manoux, M. Shipley, G. D. Batty, J. Head, M. Hamer, M. Jokela, M. Virtanen, and E. Brunner. 2011. Socioeconomic differences in cardiometabolic factors: social causation or health-related selection? Evidence from the Whitehall II Cohort Study, 1991–2004. American journal of epidemiology 174:779-789.

Evans, G. W., D. Li, and S. S. Whipple. 2013. Cumulative risk and child development. Psychological bulletin 139:1342.

Felitti, V. J., R. F. Anda, D. Nordenberg, D. F. Williamson, A. M. Spitz, V. Edwards, M. P. Koss, and J. S. Marks. 1998. Relationship of childhood abuse and household dysfunction to many of the leading causes of death in adults: The adverse childhood experiences (ACE) study. American journal of preventive medicine 14:245-258.

Harper, S. and E. C. Strumpf. 2012. Commentary: Social EpidemiologyQuestionable Answers and Answerable Questions. Epidemiology (Cambridge, Mass.) 23:795-798.

Holt-Lunstad, J., T. B. Smith, M. Baker, T. Harris, and D. Stephenson. 2015. Loneliness and social isolation as risk factors for mortality: a meta-analytic review. Perspectives on psychological science 10:227-237.

Holt-Lunstad, J., T. B. Smith, and J. B. Layton. 2010. Social Relationships and Mortality Risk: A Meta-analytic Review. PLOS Medicine 7:e1000316.

Jia, H. and E. I. Lubetkin. 2020. Impact of adverse childhood experiences on quality-adjusted life expectancy in the US population. Child Abuse & Neglect 102:104418.

Kröger, H., E. Pakpahan, and R. Hoffmann. 2015. What causes health inequality? A systematic review on the relative importance of social causation and health selection. The European Journal of Public Health 25:951-960.

Næss, Ø., B. Claussen, and G. D. Smith. 2004. Relative impact of childhood and adulthood socioeconomic conditions on cause specific mortality in men. Journal of Epidemiology & Community Health 58:597-598.

Petruccelli, K., J. Davis, and T. Berman. 2019. Adverse childhood experiences and associated health outcomes: A systematic review and meta-analysis. Child Abuse & Neglect 97:104127.

Snyder-Mackler, N., J. R. Burger, L. Gaydosh, D. W. Belsky, G. A. Noppert, F. A. Campos, A. Bartolomucci, Y. C. Yang, A. E. Aiello, A. O’Rand, K. Mullan Harris, C. A. Shively, S. C. Alberts, and J. Tung. 2020. Social determinants of health and survival in humans and other animals. Science 368.

Warren, J. R. 2009. Socioeconomic status and health across the life course: a test of the social causation and health selection hypotheses. Social forces 87:2125-2153.


